Kops: Safely Extending the eBPF Compilation Pipeline with Native Operations

eBPF safely extends OS kernels in domains such as networking, observability, and security. The safety comes from an in-kernel compilation pipeline where a verifier checks every program, and a kernel just-in-time compiler (JIT) translates the verified bytecode to native code. The kernel keeps the JIT simple to stay trustworthy, translating one bytecode instruction at a time in a single pass. This single-pass design misses optimization opportunities, so eBPF runs up to twice as slow as natively compiled code in our characterization. Adding optimizations to the kernel JIT directly requires upstream acceptance and a long release cycle, enlarges the trusted computing base (TCB), and grows the per-architecture kernel code. To address this, we present Kops, an extension interface that lets userspace compilers and kernel modules introduce new operations without modifying the kernel core, while keeping a minimal trusted computing base (TCB). Each operation has two forms, a proof sequence of vanilla eBPF instructions that the existing verifier checks and a native emit of machine instructions that the JIT compiles. Because the verifier checks the proof sequence, the native emit is the only per-operation addition to the TCB. Hardware idioms are the lowest-hanging fruit for this interface. With Kops, we build EInsn, seven operations such as rotate and conditional select that CPUs execute as single instructions. Lean 4 proofs show that each native emit computes the same result as its proof sequence. On x86-64 and ARM64, EInsn speeds up eBPF microbenchmarks by up to 24% and production applications by up to 12%. The same interface also supports whole-program native replacement, reaching 2.358x at the cost of a larger TCB.

==> figures/sec-3-perf-gap.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=\columnwidth]{figures/sec-3-perf-gap-fig.pdf}
\caption{Geometric mean of execution time per benchmark category for the eBPF JIT compiler relative to native code (LLVM \texttt{-O2}). The 54 benchmarks span seven categories: ALU/bit operations, memory access, control flow, dependency chains, loops, program scale, and code cloning.}
\label{fig:perf-gap}
\end{figure}

==> figures/sec-3-pure-bytecode-aggregate.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=\columnwidth]{figures/sec-3-pure-bytecode-aggregate-20260606.pdf}
\caption{Aggregate pure-bytecode microbenchmark speedup over kernel eBPF JIT. x86 KVM and ARM64 AWS both include kernel native, userspace eBPF, and userspace native. Higher is better; the dashed line is parity.}
\label{fig:char-pure-aggregate}
\end{figure}


==> figures/sec-6-app-case-studies.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=\columnwidth]{figures/sec-6-app-case-studies-fig.pdf}
\caption{Application-level \lang{} throughput over the stock kernel eBPF JIT.
Cilium (x86-64) compares the full policy with a single-family ablation;
Katran (ARM64) compares a conservative policy with a coverage-max policy.
Higher is better; values below 1$\times$ indicate a regression.}
\label{fig:app_case_studies}
\end{figure}


==> figures/sec-6-kinsn-micro-arm64.tex <==
\begin{figure*}[t]
\centering
\includegraphics[width=\textwidth]{figures/sec-6-arm64-kinsn-micro-rejit-20260606-backup.pdf}
\caption{ARM64 AWS matched \lang{} ReJIT microbenchmark follow-up for the selector-fixed pure-bytecode full suite. Bars report \texttt{kernel}/\texttt{kernel\_rejit} speedup from median \texttt{exec\_ns} across three samples. Green bars applied \lang{} sites; gray bars applied none. The all-29 geomean is 1.208$\times$, and the \lang{}-bearing geomean is 1.222$\times$ over 27 benchmarks.}
\label{fig:eval-kinsn-micro-arm64-old}
\end{figure*}


==> figures/sec-6-kinsn-micro-x86.tex <==
\begin{figure*}[t]
\centering
\includegraphics[width=\textwidth]{figures/sec-6-x86-kinsn-micro-best-raw-20260606-backup.pdf}
\caption{ARM64 \lang{} ReJIT speedup over the stock kernel eBPF JIT on 29
pure-bytecode microbenchmarks. Bars report \texttt{kernel}/\texttt{kernel\_rejit}
speedup; higher is better. Green bars denote benchmarks with applied \lang{}
sites. \lang{} reaches a 1.208$\times$ all-suite geomean speedup.}
\label{fig:eval-kinsn-micro-x86-old}
\end{figure*}


==> tables/sec-2-bytecode-comparison.tex <==
\begin{table}[t]
\centering
\small
\caption{Comparison of bytecode systems by verification requirements and optimization scope.}
\label{tab:bytecode-comparison}
\begin{tabular}{@{}lll@{}}
\toprule
System & Per-opcode verification & Optimization scope \\
\midrule
LLVM & None & Full \\
JVM & Type rules & Full \\
Wasm & Type + structural rules & Cross-instruction \\
eBPF & Abstract transfer function & Per-instruction \\
\bottomrule
\end{tabular}
\end{table}


==> tables/sec-3-micro-artifacts.tex <==
\begin{table*}[t]
\centering
\scriptsize
\caption{Authoritative pure-bytecode microbenchmark artifacts used for the eBPF-hardware gap characterization. Artifact suffixes identify the result directories under \texttt{micro/results}. Correctness mismatches count expected-result or retval mismatches across all recorded samples.}
\label{tab:char-micro-artifacts}
\begin{tabular}{@{}llllr@{}}
\toprule
Platform & Suite & Artifact suffix & Runtimes & Mismatches \\
\midrule
x86-64 KVM & Pure bytecode 29 & \texttt{210952\_650695} & kernel, LLVM-BPF, native, kernel native & 0 \\
ARM64 AWS & Pure bytecode 29 & \texttt{063319\_954947} & kernel, LLVM-BPF, native, kernel native & 0 \\
\bottomrule
\end{tabular}
\end{table*}


==> tables/sec-6-RQ2-RQ3.tex <==
\begin{table}[t]
\centering
\caption{Application-level \lang{} policy probes. Rows are paired by
application: Cilium compares the full policy with a single-family ablation,
while Katran compares a conservative policy with a coverage-max policy.
Workload ratios report end-to-end datapath throughput; higher is better.}
\label{tab:app_case_studies}
\small
\begin{tabular}{lcc}
\toprule
Configuration & Sites & Throughput $\uparrow$ \\
\midrule
Cilium (Full \lang{}) &
4086 &
1.074$\times$ \\

Cilium (No Bulk) &
3512 &
1.114$\times$ \\

Katran (Conservative) &
21 &
1.073$\times$ \\

Katran (Coverage-Max) &
62 &
0.995$\times$ \\
\bottomrule
\end{tabular}
\end{table}

==> tables/sec-6-kinsn-case-studies.tex <==
\begin{table*}[t]
\centering
\small
\caption{Production case studies for Cilium and Katran. Workload speedup reports post-ReJIT throughput normalized to baseline. BPF cost reports post-ReJIT per-program cost normalized to baseline, so lower is better.}
\label{tab:eval-kinsn-case-studies}
\begin{tabular}{@{}llllcccl@{}}
\toprule
Case & Platform & Policy & Sites & Workload & BPF cost & Retained / W-L-T & Dominant applied families \\
\midrule
Cilium & x86-64 KVM & Full & 4697 & 1.114$\times$ & 0.776$\times$ & 2 / 2-0-0 & lea, endian, prefetch, bulk, select \\
Katran & x86-64 KVM & No bulk & 77 & 1.032$\times$ & 0.932$\times$ & 1 / 1-0-0 & lea, rotate, endian, prefetch, extract \\
Katran & ARM64 AWS & Conservative & 21 & 1.073$\times$ & 0.941$\times$ & 1 / 1-0-0 & rotate, extract \\
\bottomrule
\end{tabular}
\end{table*}


==> tables/sec-6-kinsn-micro.tex <==
\begin{table*}[t]
\centering
\scriptsize
\caption{\lang microbenchmark evaluation artifacts. The x86 row is a local LLVM-\lang candidate against a stock-kernel baseline and is not a matched compiler-control comparison. The ARM64 row is a matched \texttt{kernel}/\texttt{kernel\_rejit} ReJIT comparison.}
\label{tab:eval-kinsn-micro}
\begin{tabular}{@{}lllccc@{}}
\toprule
Platform & Comparison & Cases & Mism. & Geomean & Sites \\
\midrule
x86-64 KVM & LLVM-\lang candidate / stock kernel & 29 & 0 & 1.216$\times$ & n/a \\
ARM64 AWS & \texttt{kernel} / \texttt{kernel\_rejit} & 29 & 0 & 1.208$\times$ & 308/308 \\
\bottomrule
\end{tabular}
\end{table*}

